Fairness-Aware Online Meta-learning

In contrast to offline working fashions, two research paradigms are devised for online learning: (1) Online Meta Learning (OML) learns good priors over model parameters (or learning to learn) in a sequential setting where tasks are revealed one after another. Although it provides a sub-linear regret bound, such techniques completely ignore the importance of learning with fairness which is a significant hallmark of human intelligence. (2) Online Fairness-Aware Learning. This setting captures many classification problems for which fairness is a concern. But it aims to attain zero-shot generalization without any task-specific adaptation. This therefore limits the capability of a model to adapt onto newly arrived data. To overcome such issues and bridge the gap, in this paper for the first time we proposed a novel online meta-learning algorithm, namely FFML, which is under the setting of unfairness prevention. The key part of FFML is to learn good priors of an online fair classification model's primal and dual parameters that are associated with the model's accuracy and fairness, respectively. The problem is formulated in the form of a bi-level convex-concave optimization. Theoretic analysis provides sub-linear upper bounds for loss regret and for violation of cumulative fairness constraints. Our experiments demonstrate the versatility of FFML by applying it to classification on three real-world datasets and show substantial improvements over the best prior work on the tradeoff between fairness and classification accuracy

==> App_proofLemma.tex <==
\begin{proof}
Following the Assumption \ref{assmp3} and analysis of the Lemma 2 in \cite{OGDLC-2012-JMLR}, we derive
\begin{align*}
    &\mathcal{L}_t(\boldsymbol{\theta}_t,\boldsymbol{\lambda}) - \mathcal{L}_t(\boldsymbol{\theta},\boldsymbol{\lambda}_t) \leq \frac{1}{2\eta_2}\Big(||\boldsymbol{\theta}-\boldsymbol{\theta}_t||^2+||\boldsymbol{\lambda}-\boldsymbol{\lambda}_t||^2\\
    &-||\boldsymbol{\theta}-\boldsymbol{\theta}_{t+1}||^2-||\boldsymbol{\lambda}-\boldsymbol{\lambda}_{t+1}||^2 \Big) + \frac{\eta_2}{2}\Big(\underbrace{||\nabla_{\boldsymbol{\theta}}\mathcal{L}_t(\boldsymbol{\theta}_t,\boldsymbol{\lambda}_t)||^2}_{\textbf{First Term (FT)}}\\
    &+\underbrace{\nabla_{\boldsymbol{\lambda}}\mathcal{L}_t|\boldsymbol{\theta}_t,\boldsymbol{\lambda}_t||^2}_{\textbf{Second Term (ST)}}\Big) - \frac{\mu_f}{2}||\boldsymbol{\theta}-\boldsymbol{\theta}_t||^2
\end{align*}
We bound FT and ST using the inequality $(a_1+a_2+\cdots+a_n)^2\leq n(a_1^2+a_2^2+\cdots+a_n^2)$. 
% As for the regularization term $\mathcal{F}(\boldsymbol{\theta})$, it simply takes the Euclidean norm $||\boldsymbol{\theta}||$.
\begin{align*}
    \text{FT}
    \leq &||\Big\langle\nabla_{\boldsymbol{\theta}'}f(\boldsymbol{\theta}'_t),\nabla_{\boldsymbol{\theta}}\mathcal{A}lg(\boldsymbol{\theta}_t)\Big\rangle+\sum_{i=1}^m\lambda_{t,i}\Big\langle\nabla_{\boldsymbol{\theta}'}g_i(\boldsymbol{\theta}'_t),\\
    &\nabla_{\boldsymbol{\theta}}\mathcal{A}lg(\boldsymbol{\theta}_t)\Big\rangle
    % +\zeta
    ||^2\\
    \leq&\Big(G(1-\eta_1 H(1+\sum_{i=1}^m\lambda_{t,i}))(1+\sum_{i=1}^m\lambda_{t,i})+\zeta\Big)^2\\
    \leq&4G^2\eta_1^2 H^2(m+1)^2(1+||\boldsymbol{\lambda}_t||^4)+2\zeta^2
\end{align*}
and the second term
\begin{align*}
    \text{ST}
    \leq&||\Big\{\Big\langle\nabla_{\boldsymbol{\theta}'}f(\boldsymbol{\theta}'),\nabla_{\boldsymbol{\lambda}}\mathcal{A}lg(\boldsymbol{\theta})\Big\rangle+\sum_{i=1}^m\Big(g_i(\boldsymbol{\theta}')+\\
    &\lambda_{t,i}\Big\langle\nabla_{\boldsymbol{\theta}'}g_i(\boldsymbol{\theta}'),\nabla_{\boldsymbol{\lambda}}\mathcal{A}lg(\boldsymbol{\theta})\Big\rangle-\delta\eta_2\lambda_{t,i}\Big)\Big\}||^2\\
    \leq&\Big(\sum_{i=1}^m(D-\lambda_{t,i}G^2\eta_1 m -\delta\eta_2\lambda_{t,i} -\eta_1G^2)\Big)^2\\
    \leq&4m(D^2+G^4\eta_1^2m^2||\boldsymbol{\lambda}_t||^2+\delta^2\eta_2^2||\boldsymbol{\lambda}_t||^2+\eta_1^2G^4)
\end{align*}
By adding the inequalities of FT and ST, and using the fact $||\boldsymbol{\theta}||\leq R$ and $t\geq 1$ we complete the proof.
\end{proof}

==> fairness.tex <==
Intuitively, an attribute affects the target variable if one depends on the other. Strong dependency indicates strong effects. In general, group fairness criteria used for evaluating and designing machine learning models focus on the relationships between the protected attribute and the system output. Therefore, the problem of group unfairness prevention can be seen as a constrained optimization problem. For simplicity, we consider one binary protected attribute (\textit{e.g.} white and black) in this work. However, our ideas can be easily extended to many protected attributes with multiple levels.

Let $\mathcal{Z=X\times Y}$ be the data space, where $\mathcal{X} = \mathcal{E} \cup\mathcal{S}$. Here $\mathcal{E} \subset \mathbb{R}^d$ is an input space, $\mathcal{S} = \{0,1\}$ is a protected space, and $\mathcal{Y} = \{0,1\}$ is an output space for binary classification. At each round $t\in[T]$, for each task $k\in[t-1]$, we let $\{\mathbf{e}_{k,i}, y_{k,i}, s_{k,i}\}_{i=1}^n \in(\mathcal{E\times Y\times S})$ be the corresponding task data and $n$ is the number of datapoints in the support set. In referencing fairness, we are using same amount of training examples irrespective of class label, with the assumption that all tasks are 2-way. A fine-grained measurement to ensure fairness in class label prediction is to design fair classifiers by controlling the decision boundary covariance (DBC) \cite{Zafar-AISTATS-2017}.
\begin{definition}[Decision Boundary Covariance \cite{Zafar-AISTATS-2017}]
The covariance between the protected variables $\mathbf{s}=\{s_i\}_{i=1}^n$ and the signed distance from the feature vectors to the decision boundary, $d_{\boldsymbol{\theta}} (\mathbf{e}) = \{d_{\boldsymbol{\theta}} (\mathbf{e}_i)\}_{i=1}^n$, 
% where $\mathbf{\alpha}$ is the decision boundary parameter.
\begin{align}
\label{dbc definition}
    \text{DBC}(\mathbf{s}, d_{\boldsymbol{\theta}}(\mathbf{e})) = \mathbb{E} \big[ (\mathbf{s}-\mathbf{\Bar{s}})d_{\boldsymbol{\theta}}(\mathbf{e}) \big]
\end{align}
where $\mathbf{\Bar{s}} = (\frac{1}{n}\sum_{i=1}^n s_i)\mathbbm{1}$. 
\end{definition}
Therefore, a point $\boldsymbol{\theta}$ in the domain of a task is feasible if it satisfies the fairness constraint $g(\boldsymbol{\theta})\leq 0$. More concretely, $g(\boldsymbol{\theta})$ is defined by the definition of DBC in Eq.(\ref{dbc definition}), \textit{i.e.}
\begin{align}
\label{eq:DBC constraint}
    g(\boldsymbol{\theta}) = \Big| {\frac{1}{n}\sum\nolimits_{\mathbf{s,e}\sim\mathcal{D}, i=1}^n(s_i-\Bar{s})d_{\boldsymbol{\theta}}(\mathbf{e}_i)} \Big| -\epsilon
\end{align}

where $\epsilon$ is a small positive fairness relaxation. To formalize the supervised classification problem in the context of meta-learning definitions, a cross-entropy loss function is used to describe the adapted loss over a support set for each task.
